The RaspGrade Dataset: Towards Automatic Raspberry Ripeness Grading with Deep Learning

This research investigates the application of computer vision for rapid, accurate, and non-invasive food quality assessment, focusing on the novel challenge of real-time raspberry grading into five distinct classes within an industrial environment as the fruits move along a conveyor belt. To address this, a dedicated dataset of raspberries, namely RaspGrade, was acquired and meticulously annotated. Instance segmentation experiments revealed that accurate fruit-level masks can be obtained; however, the classification of certain raspberry grades presents challenges due to color similarities and occlusion, while others are more readily distinguishable based on color. The acquired and annotated RaspGrade dataset is accessible on Hugging Face at: https://huggingface.co/datasets/FBK-TeV/RaspGrade.

==> Tables/sota.tex <==
%%%%%%%%%%%%%%%%%%%%%%TABLE MV%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[!htbp]
\captionsetup{size=footnotesize}
\caption{Summary of MV Technologies}
\setlength\tabcolsep{3pt} % let LaTeX compute intercolumn whitespace
\setlength{\extrarowheight}{5pt} % Add extra height to each row
\newcolumntype{C}[1]{>{\raggedright\arraybackslash}p{#1}} %To center align a particular column
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}} %To left align a particular column
\scriptsize\centering
\smallskip 
\begin{tabular}{C{2cm}C{2.5cm}C{2.5cm}L{2.5cm}C{4.5cm}C{2cm}}
\toprule
% \textbf{Product} & \textbf{Task} & \textbf{Sensor} & \textbf{Illumination} & \textbf{Software}  & \textbf{Ref. }\\
Product & Task & Sensor & Illumination & Software & Reference\\
\midrule  

Apple & Detection  & Thermal & Halogen lamp with filters to diffuse light & Texture features and Support vector machine & \cite{multispectral} \\
Onions & Estimate the weight, diameter and volume & Multimodal (color, hyperspectral, 3D, and X-ray) & Fluorescent lamps & Support vector machine with radial basis function & \cite{wang2015multimodal} \\
Citrus fruit & Counting & RGB & N/A & Retinex algorithm for image enhancement, Logistic and KNN and Bayesian classifiers (i.e., Citrus vs background) and Watershed algorithm for Citrus segmentation & \cite{rgb1} \\
Atlantic salmon & Grading based on wound and deformity & Three color CMOS cameras & LED strips containing multiple LED &  Color and geometric features and Support vector machine with radial basis kernel & \cite{sture20163d} \\
Olives & Detection based on the skin health condition  & RGB and multi-Spectral & N/A & Edge detection and segmentation via connected components algorithm & \cite{infrared} \\
Tuna and Salmon meat & Freshness classification & RGB & LED & Color historgrams and AutoML machine learning models & \cite{medeiros2021computer}\\
Salmon and rainbow trout & Slaughtering & Line-scan laser
triangulation system & N/A & 3D fish segmentation, median filtering for noise removal,  geometric feature extraction for head/tail classification and Incision-point determination with linear discriminant analysis & \cite{steen2011automated} \\
Chicken pieces & Sorting & RGB & Linear LED tubes & Otsu method for segmentation, shape/colour/texture feture extraction, Chi-Square algorithm for dimensionality reduction, Partial least squares regression and Linear discriminant analysis and Artificial neural network models were used for classification & \cite{teimouri2018line}\\
Eggs & Sorting & RGB & LED & Connected components for egg segmentation and geometric feature extraction for threshold-based sorting & \cite{vasileva2018assessing} \\
Chicken meat & Springiness prediction & Hyperspectral &  Halogen lamps & Partial least square regression and artificial neural networks for prediction & \cite{xiong2015application} \\
Beef and lamb & Grading & RGB & LED & Texture descriptors and Partial Least Squares & \cite{stewart2021objective} \\


\bottomrule
\end{tabular}
\label{table1}
\end{table*}
\normalsize

\normalsize


